Graphite: A GPU-Accelerated Mixed-Precision Graph Optimization Framework

We present Graphite, a GPU-accelerated nonlinear least squares graph optimization framework. It provides a CUDA C++ interface to enable the sharing of code between a real-time application, such as a SLAM system, and its optimization tasks. The framework supports techniques to reduce memory usage, including in-place optimization, support for multiple floating point types and mixed-precision modes, and dynamically computed Jacobians. We evaluate Graphite on well-known bundle adjustment problems and find that it achieves similar performance to MegBA, a solver specialized for bundle adjustment, while maintaining generality and using less memory. We also apply Graphite to global visual-inertial bundle adjustment on maps generated from stereo-inertial SLAM datasets, and observe speed-ups of up to 59x compared to a CPU baseline. Our results indicate that our framework enables faster large-scale optimization on both desktop and resource-constrained devices.

==> tables/specs.tex <==
\begin{table}[t]
    \caption{Evaluation machine specifications.}
    \label{tab:specs}
    \centering
    \begin{tabular}{c|cc}
         \bf Machine & \bf Specs\\
         \hline
         & 12-core Intel Core i7-12700K CPU @ 3.8-4.9 GHz\\ %3.8-4.9 GHz\\
         Desktop & 10496-core NVIDIA RTX 3090 GPU @ 1.9 GHz\\
        & 64 GB RAM\\ 
         \hline
        & 6-core ARM Cortex-A78AE CPU @ 1.7 GHz \\
        Orin Nano & 1024-core NVIDIA Ampere GPU @ 1.0 GHz \\
        & 8 GB RAM\\
         \hline
    \end{tabular}
    % \vspace{-20pt}
\end{table}
